Transformers versus the EM Algorithm in Multi-class Clustering

LLMs demonstrate significant inference capacities in complicated machine learning tasks, using the Transformer model as its backbone. Motivated by the limited understanding of such models on the unsupervised learning problems, we study the learning guarantees of Transformers in performing multi-class clustering of the Gaussian Mixture Models. We develop a theory drawing strong connections between the Softmax Attention layers and the workflow of the EM algorithm on clustering the mixture of Gaussians. Our theory provides approximation bounds for the Expectation and Maximization steps by proving the universal approximation abilities of multivariate mappings by Softmax functions. In addition to the approximation guarantees, we also show that with a sufficient number of pre-training samples and an initialization, Transformers can achieve the minimax optimal rate for the problem considered. Our extensive simulations empirically verified our theory by revealing the strong learning capacities of Transformers even beyond the assumptions in the theory, shedding light on the powerful inference capacities of LLMs.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{claim}{Claim}
\newtheorem{algo}{Procedure}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{question}{Question}
\newtheorem{fact}{Fact}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{mytheorem}{Theorem}
\numberwithin{mytheorem}{section}
\newtheorem{mylemma}{Lemma}
\numberwithin{mylemma}{section}
\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{%
  \newenvironment{#1}[1]
  {%
   \renewcommand\customgenericname{#2}%
   \renewcommand\theinnercustomgeneric{##1}%
   \innercustomgeneric
  }
  {\endinnercustomgeneric}
}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\p}[1]{#1^{\prime}}
\newcommand{\scr}[1]{\mathscr{#1}}
\newcommand{\h}[1]{\hat{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\hti}[1]{\hat{\tilde #1}}
\newcommand{\bfa}[1]{\boldsymbol{#1}}
\newcommand{\fk}[1]{\mathfrak{#1}}
\DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
\newcommand{\ca}[1]{\pazocal{#1}}
\newcommand{\mca}[1]{\mathcal{#1}}
\newcommand{\mtt}[1]{\mathtt{#1}}
\newcommand{\zt}{{Z_{\ca T}}}
\newcommand{\nnb}{\nonumber}
\newcommand{\ezt}{{\ca Z_{\ca T}}}
\newcommand{\sn}[1]{{S}_h^{(#1)}}
\newcommand{\tz}[1]{\fk S_{#1}}
\newcommand{\tzp}[1]{\fk S^i_{#1}}
\newcommand{\bbm}[1]{\mathbbm {#1}}
\newcommand{\bscr}[1]{\bar{\scr #1}}
\newcommand{\dtz}[2]{\fk S^{#1}_{#2}}
\newcommand{\ewt}[2]{\bb E[\Vert\delta^i\bfa w_{#1}\Vert^{#2}]}
\newcommand{\vwt}[1]{Var[\Vert\delta^i\bfa w_{#1}\Vert]}
\newcommand{\wt}[1]{\Vert\delta^i\bfa w_{#1}\Vert}
\newcommand{\rmg}{R^{(m)}(h_{\ca G})}
\newcommand{\emrr}[1]{\wh R_{#1}(h_{#1})}
\newcommand{\wrg}[1]{\wh R(h_{\ca G_{#1}})}
\newcommand{\st}[1]{{#1}^*}
\newcommand{\prox}{\text{prox}}
\newcommand{\stp}[1]{{#1}^{*\prime}}
\newcommand{\stpb}[1]{{\bfa #1}^{*\prime}}
\newcommand{\bell}{(\ell)}
\newcommand{\tdas}{\tda^{*}}
\newcommand{\pr}[1]{{#1}^\prime}
\newcommand{\hsp}{h^{\mathtt{sparse}}}
\newcommand{\spm}{S^\prime}
\newcommand{\dmax}{{d_{\max}}}
\newcommand{\tprime}{\prime\prime\prime}
\newcommand{\emr}[1]{\wh R_{\ca Z^{#1}}(h_{\ca Z^{#1}})}
\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mr}[1]{ R(h_{\ca Z^{#1}})}
\newcommand{\bbem}{\bb E_{\ca Z_1^m\sim\bb D^m}}
\newcommand{\bbemt}{\bb E_{\ca Z_1^m,\ca Z^\text{test}\sim\bb D^{m+1}}}
\newcommand{\tet}{\text{test}}
\newcommand{\wha}[1]{\wh{\bfa #1}}
\newcommand{\rank}{\mathtt{rank}}
\newcommand{\lef}{\left}
\newcommand{\rig}{\right}
\newcommand{\dw}{\Vert\delta^i\bfa w_t\Vert}
\newcommand{\dwt}{\Vert\delta^i\bfa w_T\Vert}
\newcommand{\tda}[1]{\tilde{\bfa{#1}}}
\newcommand{\tv}{\mathtt{TV}}
\newcommand{\xb}{\bfa{X\beta}}
\newcommand{\bx}{\bfa\beta^\top\bfa X^\top}
\newcommand{\bta}[1]{\bfa{#1}^\top}
\newcommand{\sgmx}{\bfa\Sigma_x}
\newcommand{\lsts}{\ell_{s,t}^*}
\newcommand{\Lsts}{\ca L_{s,t}^*}
\newcommand{\lits}{\lambda_{i,t,\lambda^*}}
\newcommand{\liss}[1]{\lambda_{i,#1,\lambda^*}}
\newcommand{\ts}{\theta_S}
\newcommand{\TS}{\Theta_S}
\newcommand{\tdx}{\tilde x}
\newcommand{\td}{\tau_\delta}
\newcommand{\vect}{\text{vec}}
\newcommand{\vca}{\vect(A)}
\newcommand{\vcb}{\vect(B)}
\newcommand{\pta}{\partial}
\newcommand{\proja}{\mathtt{proj_A}}
\newcommand{\projb}{\mathtt{proj_B}}
\newcommand{\mbbm}[1]{\mathbbm{#1}}
\newcommand{\tths}{\tilde{\theta}_S}
\newcommand{\bs}{B_S}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\tint}{\text{int}}
\newcommand{\dom}{\text{dom}}
\newcommand{\as}{A_S}
\newcommand{\ths}{\theta_S}
\newcommand{\tde}{\tilde}
\newcommand{\pri}{\prime}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\diag}{\text{diag}}
\newcommand{\onen}[1]{\Vert#1\Vert_1}
\newcommand{\fron}[1]{\Vert#1\Vert_F}
\newcommand{\fnor}{\fron}
\newcommand{\ve}[1]{\vect \lef (#1\rig )} 
\newcommand{\twon}[1]{\lef\Vert #1\rig\Vert_2}
\newcommand{\ub}[1]{\underbrace{#1}}
\newcommand{\ob}[1]{\overbrace{#1}} 
\newcommand{\tas}{\tde A_S}
\newcommand{\tbs}{\tde B_S}
\newcommand{\sas}{\tde A^*_S}
\newcommand{\sbs}{\tde B^*_S}
\newcommand{\laminus}{\Vert\lambda_{S}^{*\odot -1}\Vert_2}
\newcommand{\laplus}{\Vert\lambda^*\Vert_2}
\newcommand{\ptaa}{\lef\Vert\frac{\pta\lambda_{S,t}}{\pta\ve A^\prime}\rig\Vert}
\newcommand{\ptab}{\lef\Vert\frac{\pta\lambda_{S,t}}{\pta\ve B^\prime}\rig\Vert}
\newcommand{\lats}{\lambda_{S,t}^{\#*\odot -1}}
\newcommand{\lato}{\lambda_{S,t}^{*\odot-1}}
\newcommand{\xiosq}{\tde x_i^{\odot 2}}
\newcommand{\xissq}{\tde x_i^{\#\odot 2}}
\newcommand{\lstl}[2]{\lambda_{S,#1}^{*\odot-#2}}
\newcommand{\xst}[1]{\tdx_{S,#1}^{\odot 2}}
\newcommand{\otwo}{{\odot 2}}
\newcommand{\oone}{{\odot 1}}
\newcommand{\tso}{\theta_{1,S}}
\newcommand{\tst}{\theta_{2,S}}
\newcommand{\tsth}{\theta_{3,S}}
\newcommand{\vas}[1]{\ve{A_{#1,S}}}
\newcommand{\vbs}[1]{\ve{B_{#1,S}}}
\newcommand{\losso}{\ca L^*_s}
\newcommand{\lossp}{\ca L_s}
\newcommand{\tr}{\text{Tr}}
\newcommand{\tsss}{\theta_S^{***}}
\newcommand{\trc}{\theta_{\ca R^c}}
\newcommand{\elst}{\ell_{s,t}}
\newcommand{\whtss}{\wh{\theta}_S^*}
\newcommand{\pz}[1]{\psi_{\zeta_{ #1}}}
\newcommand{\qz}[1]{q_{\zeta_{ #1}}}
\newcommand{\whts}{\wh\theta_S}
\newcommand{\whtr}{\wh\theta_{\ca R}}
\newcommand{\whtsr}{\wh\theta_S^{*r}}
\newcommand{\tro}{\theta_{\ca R,1}}
\newcommand{\tthr}{\tde\theta_{\ca R}}
\newcommand{\whtsss}{\wh\theta_S^{***}}
\newcommand{\hlt}{\wh\lambda^{*t}}
\newcommand{\hks}{\ca H_{k,S_0}}
\newcommand{\bl}{{\bigg (}}
\newcommand{\br}{{\bigg )}}
\newcommand{\whtrss}{\wh\theta_{\ca R}^{***}}
\newcommand{\diagone}{\diag\lef(-\lambda_{S,t}^{\odot-2}+2\lambda_{S,t}^{\odot-3}\odot\tde x_{S,t}^{\odot 2}\rig)}
\newcommand{\vtl}{\Vert\lambda_t\Vert}
\newcommand{\bern}{\text{Bern}}
\newcommand{\Uniform}{\text{Uniform}}
\newcommand{\diagtwo}{\lambda_{S,t}^{\odot -1}-\lambda_{S,t}^{\odot -2}\odot\tde x_{S,t}^{\odot 2}}
\newcommand{\md}{\text{maxdeg}}
\newcommand{\rfcw}{\text{RFCW}}
\newcommand{\Null}{\text{Null}}
\newcommand{\tid}[1]{\tde{\hat #1}}
\newcommand{\sm}[1]{\small{#1}\normalsize}
\newcommand{\tny}[1]{\footnotesize{#1}\normalsize}
\newcommand{\ttny}[1]
{\scriptsize{#1}\normalsize}
\newcommand{\tttny}[1]{\tiny{#1}\normalsize}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\pink}[1]{\textcolor{pink}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/appenda.tex <==
\section{Theoretical Background}
This section provides approximation results of the Softmax function in the form of $f(\bfa x):=\sum_{i=1}^M a_i\sigmoid\lef(\bfa x^\top\bfa v_i\rig)+a_0$ where $\{a_i\}_{i\in[M]}\subset \bb R$ and $\{\bfa v_i\}\subset \bb R^{d+1}$. We consider the class of $(R, C_{\ell})$-smooth functions \citep{bach2017breaking,bai2024transformers} defined as follows.
\begin{definition}[\citet{bai2024transformers}]\label{rcsmoothfunc}
    A function $g:\bb R^d\to\bb R$ is $(R, C_{\ell})$ smooth if for $s= \lceil(k-1)/2\rceil+2$, $g$ is a $C^s$ function supported on $[-R, R]^k$ such that
    \begin{align*}
        \sup_{\bfa x\in [-R,R]^k}\Vert\nabla^ig(\bfa x)\Vert_{\infty}\leq L_i,
    \end{align*}
    for all $i\in\{0,1,\ldots,s\}$, with $\max_{0\leq i\leq s}L_iR^i\leq C_{\ell}$.
\end{definition}
We then consider the following class of functions
\begin{align*}
    &\ca F_d = \bigg\{f:f(\bfa x)=\int_{\ca W:\Vert\bfa v\Vert=1}\sigmoid\lef([\bfa x^\top,1]\bfa v\rig)d\mu(\bfa v)\bigg\},\text{ with } TV(\mu)=\int_{\ca W:\Vert\bfa v\Vert_2=1}d|\mu(\bfa v)|<C_{\ell}C(f)^d ,
\end{align*}
where $C(f)$ is a constant that depends only on $f$. 
It is further noted that by \citet{bach2017breaking}, we can write that the class of $(R, C_{\ell})$ smooth functions belongs to the above class. Then we prove the following approximation lemma for the sigmoid function, which provides explicit dependence on $B$ and $C$.
 \begin{lemma}\label{sigmoidapprox}
     Suppose $f$ is $(R,C_{\ell})$ smooth. Then there exists a set of points $(\bfa v_1, a_1),\ldots,(\bfa v_M, a_M)\in \ca B(\Vert\cdot\Vert_2, 1)$ that makes the following hold
     \begin{align*}
         \sup_{\bfa x\in \ca B\lef(\Vert\cdot\Vert_\infty,R\rig)}\Big|\frac{1}{C_{\ell}}f(\bfa x)-\frac{1}{M}\sum_{i=1}^Ma_i\sigmoid\lef([\bfa x^\top,1]^\top\bfa v_i\rig)\Big|&\leq  C(f)^d\inf_{\epsilon>0}\Big(2\epsilon+\sqrt{\frac{\log(\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)/\delta)}{M}}\Big)\\
         &\lesssim C(f)^d\sqrt{\frac{d}{M}\log\Big(\frac{MR}{d}\Big)},
     \end{align*}
     where we also have $\sum_{i=1}^M|a_i|\leq C(f)^d$.
 \end{lemma}
 \begin{proof}
     The proof goes by the probabilistic method, where we can first use \citet{pisier1981remarques} to show that when we sample from the distribution given by $f(\bfa v)=\frac{|\mu(\bfa v)|}{\int_{\bb S^d}d\mu(\bfa v)}=\frac{|\mu(\bfa v)|}{TV(\mu)}$. Then, under this probability measure, we sample independently in a total of $M$ samples $(\bfa V_1, \ldots, \bfa V_M)$ to obtain that for any $\bfa x\in\ca V$, pointwise
     \begin{align*}
         \int_{\bb R^{d+1}}&\softmaxx\lef([\bfa x^\top, 1]\bfa v\rig)d\mu(\bfa v)- \frac{TV(\mu)}{M}\sum_{i=1}^M\softmaxx\lef([\bfa x^\top, 1]\bfa V_i\rig)\\
         &= TV(\mu)\bl\bb E\Big[\sign(\mu(\bfa v)) \softmaxx\lef([\bfa x^\top,1]\bfa V\rig)\Big]-\frac{1}{M}\sum_{i=1}^M\sign\lef(\mu(\bfa v)\rig)\softmaxx\lef([\bfa x^\top,1]\bfa V_i\rig)\br.
     \end{align*}
     And we have by Hoeffding's inequality,
     \begin{align*}
         \bb P\bl\Big|\bb E\lef[\sign(\mu(\bfa v))\softmaxx\lef([\bfa x^\top, 1]\bfa V\rig)\rig]-\frac{1}{M}\sum_{i=1}^M\sign(\sigma_f(\bfa V_i))\softmaxx\lef([\bfa x^\top, 1]\bfa V_i\rig)\Big|\geq \frac{t}{TV(\mu)}\br\leq\exp\lef(-\frac{CMt^2}{TV(\mu)^2}\rig).
     \end{align*}
     And, by the union bound, we can show that for points in the $\epsilon$-cover of $\ca B(\Vert\cdot\Vert_{\infty},R)$, the following holds
     \begin{align*}
         \bb P\bl\sup_{\bfa x\in \ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)}&\Big|\bb E\Big[\ub{\sign(\sigma_f (\bfa V))\softmaxx\lef([\bfa x^\top, 1]\bfa V\rig)}_{=:F(\bfa V,\bfa x)}\Big]-\frac{1}{M}\sum_{i=1}^M\sign(\sigma_f(\bfa V_i))\softmaxx\lef([\bfa x^\top,1]\bfa V_i\rig)\Big|\geq\frac{t}{TV(\mu)}\br\\
         &\leq |\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)|\exp\lef(-\frac{CMt^2}{TV(\mu)^2}\rig).
     \end{align*}
     Alternatively, we can show the following holds with probability at least $1-\delta$,
     \begin{align*}
         \sup_{\bfa x\in\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)}&\Big|\bb E\lef[\sign(\mu(\bfa v))\softmaxx\lef([\bfa x^\top,1]\bfa V\rig)\rig]-\frac{1}{M}\sum_{i=1}^M\sign(\sigma_f)\softmaxx\lef([\bfa x^\top,1]\bfa V_i\rig)\Big|\\
         &\leq \sqrt{\frac{\log\lef(\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)/\delta\rig)}{M}}.
     \end{align*}

     Then we consider generalizing these results to uniform convergence. For $\bfa x$, we denote $\pi(\bfa x)$ as the closest point in the $\epsilon$-cover of $\ca B(\Vert\cdot\Vert_{\infty},R)$ denoted by $\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)$. For function $F$, we can show that for all $\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)$,
     \begin{align*}
         \sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\lef|\bb E[F(\bfa V,\bfa x)] - \bb E[F(\bfa V,\pi(\bfa x))]\rig|\leq \lef|\bfa V^\top(\bfa x_1-\bfa x_2)\rig|\leq\Vert\bb E[\bfa V^\top]\Vert_2\Vert\bfa x_1-\bfa x_2\Vert_2\leq \epsilon.
     \end{align*}
     Then we consider the error given by
     \begin{align*}
         \sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\Big|\frac{1}{M}\sum_{i=1}^MF(\bfa V_i,\bfa x)-\frac{1}{M}\sum_{i=1}^MF(\bfa V_i,\pi(\bfa x))\Big|\leq\frac{1}{M}\sum_{i=1}^M\epsilon\Vert\bfa V_i\Vert_2\leq\epsilon.
     \end{align*}
    Then the following holds with probability at least $1-\delta$,
     \begin{align*}
         &\sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\Big|\bb E\lef[F(\bfa V, \bfa x)\rig]-\frac{1}{M}\sum_{i=1}^MF(\bfa V_i,\bfa x)\Big|\\
         &\leq \sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\Big|\bb E\lef[F(\bfa V, \bfa x)\rig]-\bb E\lef[F(\bfa V, \pi(\bfa x))\rig]\Big|+\sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\Big|\frac{1}{M}\sum_{i=1}^MF(\bfa V_i,\bfa x)-\frac{1}{M}\sum_{i=1}^MF(\bfa V_i, \pi(\bfa x))\Big|\\
         &+\sup_{\pi(\bfa x)\in\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)}\Big|\bb E\lef[F(\bfa V,\pi(\bfa x))\rig]-\frac{1}{M}\sum_{i=1}^MF(\bfa V_i,\pi(\bfa x))\Big|\leq\epsilon+\epsilon + \sqrt{\frac{\log(\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon)/\delta)}{M}}.
     \end{align*}
     Given these results, we show that there exists a set of parameters $\{(\bfa V_i, a_i=TV(\mu)\sign_f(\bfa V_i))\}_{i\in[m]}$ where the following holds
     \begin{align*}
         \sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty},R)}\Big|\frac{1}{C_{\ell}}f(\bfa x)-\frac{1}{M}\sum_{i=1}^M a_i\softmaxx\lef([\bfa x^\top, 1]\bfa V_i\rig)\Big|&\lesssim \inf_{\epsilon}\bigg\{\epsilon+\sqrt{\frac{\log(\ca N(\ca B(\Vert\cdot\Vert_{\infty},R),\epsilon))}{M}}\bigg\}\\
         &\lesssim \inf_{\epsilon}\bigg\{\epsilon +\sqrt{\frac{d\log\frac{R}{\epsilon}}{M}}\bigg\}\lesssim\sqrt{\frac{d}{M}\log\lef(\frac{MR}{d}\rig)},
     \end{align*}
     where we already utilize the estimate given by \citet{wu2020information} on the covering number of $L_2$ balls.
 \end{proof}
 \begin{lemma}[Approximating $d$ Dimensional $(R, C_{\ell})$ smooth functions by Softmax Neural Networks]\label{softmaxapprox}
        Consider an element-wise $(R, C_{\ell})$ smooth mapping $\bfa f(\bfa x)=(f_1(\bfa x),\ldots f_k(\bfa x))^\top$ where $\bfa x\in[-R,R]^d$. There exists a set of points $\{(\bfa A_{i}, a_{i})\}_{i\in[M]}$ such that the following hold
        \begin{align*}
            \sup_{\bfa x\in\ca B\lef(\Vert\cdot\Vert_\infty, R\rig)}\frac{1}{C_{\ell}}\Big\Vert\bfa f(\bfa x)-\sum_{i=1}^{Md} a_i\softmaxx\lef(\bfa A_i\begin{bmatrix}
                \bfa x\\
1\end{bmatrix}\rig)\Big\Vert_{\infty}\leq C(f)^d\sqrt{\frac{d^2}{M}\log\lef(\frac{MR}{d^2}\rig)}.
        \end{align*}
 \end{lemma}
 \begin{proof}
     Our proof goes by connecting the $\softmax$ activation with the $\sigmoid$ functions. Note that by lemma \ref{sigmoidapprox} we can show that for all $\ell\in[k]$, there exists a set $\{(\bfa v_i^{(\ell)}, a_i^{(\ell)})\}_{\ell\in[M^\prime]}$
     \begin{align*}
         \sup_{\bfa x\in\ca B\lef(\Vert\cdot\Vert_{\infty}, R\rig)}\frac{1}{C_{\ell}}\Big|f_{\ell}(\bfa x)-\sum_{i=1}^{M^\prime}a_i^{(\ell)}\sigmoid\lef(\bfa v_i^{(\ell),\top}\begin{bmatrix}
             \bfa x\\
             1
         \end{bmatrix}\rig)\Big|\leq C(f)^d\sqrt{\frac{d}{M^\prime}\log\lef(\frac{M^\prime R}{d}\rig)}.
     \end{align*}
     Consider the following matrices construction of $\{\bfa B_{i}^{(\ell)}\}_{i\in[d], \ell\in[M]}\subset\bb R^{k\times d}$, given by 
            $\bfa B_{i}^{(\ell)} = \begin{bmatrix}
            \bfa 0_{(\ell-1)\times (d-1)}& 0\\
             \bfa v_{i,[d-1]}^{(\ell),\top}&\log d+\bfa v_{i,d}^{(\ell)}\\
             \bfa 0&\bfa 0
         \end{bmatrix}$. Then we can show that
         \begin{align*}
             \sup_{\bfa x\in\ca B(\Vert\cdot\Vert_{\infty})}\bigg\Vert\begin{bmatrix}
                 \bfa 0_{(\ell-1)\times 1}\\
                 f_{\ell}(\bfa x)\\
                 \bfa 0
             \end{bmatrix}-\sum_{i=1}^{M^\prime}a_i^{(\ell)}\softmaxx\lef(\bfa B_i^{(\ell)}\begin{bmatrix}
                 \bfa x\\
                 1
             \end{bmatrix}\rig)\bigg\Vert_{\infty}\leq C(f)^d\sqrt{\frac{d}{M^\prime}\log\Big(\frac{M^\prime R}{d}\Big)},
         \end{align*}
         which completes the proof through noticing that $M^\prime d=M$.
 \end{proof}
    \begin{lemma}[Norm Approximation by Sigmoid Functions]\label{Softmaxapprox1/x}
    Consider the vector $\bfa v\in\bb R^d$. Assume that there exists a constant $C$ with $\Vert\bfa v\Vert_2\leq C$. For $M<\lef(C\frac{\overline R}{\underline R}\rig)^d\frac{1}{\epsilon^2}\log(1+C/\epsilon)$ such that there exists $\{\bfa a_m\}_{m\in[M]}\subset\bb S^{d}$ and $\{c_m\}_{m\in[M]}\subset\bb R$ where for all $\bfa v$ with $\overline R\geq\Vert\bfa v\Vert_2\geq \underline R$, we have 
    \begin{align*}
        \bigg|\sum_{m=1}^Mc_m\sigmoid\lef(\bfa a_m^\top\begin{bmatrix}
            \bfa v\\
            1
        \end{bmatrix}\rig)-\frac{1}{\Vert\bfa v\Vert_2}\bigg|\leq \lef(\frac{C\overline R}{\underline R}\rig)^d\sqrt{\frac{d}{M}\log\lef(\frac{MR}{d^2}\rig)}.
    \end{align*}
    % Similarly, there exists a multihead ReLU attention layer with number of heads $M\leq\overline R^{\frac{d}{2}}\frac{C(d)}{\epsilon^2}\log\lef(1+C/\epsilon\rig)$, a set of vectors $\{\bfa b_m\}_{m\in[M]}\subset\bb S^{N-1}$ and $\{d_m\}_{m\in[M]}\subset\bb R$ such that 
    % \begin{align*}
    %     \Big|\sum_{m=1}^Md_m\sigma(\bfa b_m^\top\bfa v)-\Vert\bfa v\Vert_2^{1/2}+1\Big|\leq\epsilon.
    % \end{align*}
\end{lemma}
\begin{proof}
    Consider a set $\ca C^d(\overline R) :=\ca B^d_{\infty}(\overline R)\setminus\ca B_{2}^d(\underline R)$, we note that
    \begin{align*}
        \sup_{\bfa v\in\ca C^d(\overline R)}\pta_{v_{j_1},\ldots,v_{j_i}\in[d]}\bl\frac{1}{\Vert\bfa v\Vert_2}\br\leq\frac{C^d}{\Vert\bfa v\Vert_2^d}\leq\frac{C^d}{\underline R^d}.
    \end{align*}
    Therefore, consider the definition \ref{rcsmoothfunc}, we have $C_{\ell}=\lef(\frac{\overline R}{\underline R}\rig)^d C^d$. Then the result is concluded by lemma \ref{Softmaxapprox1/x}.
\end{proof}

%  After a careful evaluation of the proof of the above lemma, we come up with the following corollary, which provides explicit dependence on the maximum value. 
% \begin{lemma}\label{lm:a1}
%     Suppose $f\in\ca F_d^{2m}$ with $|f|<B_f$, then for all bounded sets $U\subset\bb R^d$, there exists $B(d,f,U)<\infty$
%  and a point $((\bfa v_1,a_1),\ldots(\bfa v_M,a_M))\in [\bb R^{d+1}\times[-B,B]]^{M}$ such that the following holds
%  \begin{align*}
%      \sup_{0\leq \alpha\leq m}\sup_{\bfa x\in U}\Big|D^{\alpha}f(\bfa x)-\frac{1}{M}\sum_{i=1}^Ma_iD^{\alpha}\sigmoid\lef([\bfa x^\top,1]\bfa v_i\rig)\Big|\leq B_f C(d,f,U)M^{-1/2}.
%  \end{align*}
%  \end{lemma}
% where $\mu$ is the Radon measure and $\ca V$ is a compact space and
% \begin{align*}
%     \gamma_2(f) = \inf_{p}\int_{\ca V}|p(\bfa v)|^2d\tau(\bfa v),\quad\text{ s.t. }f(\bfa x)=\int_{\ca V}p(\bfa v)\sigmoid(\bfa v^\top\bfa x)d\tau(\bfa v),
% \end{align*}
% with $\tau$ being a fixed probability measure. Then, we employ the result coming from \citet{bach2017breaking,bai2024transformers} and consider the following smooth function class.
% \begin{definition}[Sufficiently smooth $d$-variate function] We say a function $g:\bb R^d\to\bb R$ is $(R,C_{\ell})$-smooth if for $s=\lceil (d-1)/2\rceil+2$, $g$ is a $C^s$ function on $\ca B_{\infty}^d(R)$, and
% \begin{align*}
%     \sup_{z\in\ca B_{\infty}^d(R)}\Vert\nabla^i g(\bfa z)\Vert_{\infty}=\sup_{\bfa z\in\ca B_{\infty}^d(R)}\max_{j_1,\ldots, j_i\in[d]}\lef|\partial_{x_{j_1}\ldots x_{j_i}}g(\bfa x)\rig|\leq L_i
% \end{align*}
% for all $i\in\{0,1,\ldots, s\}$ with $\max_{0\leq i\leq s}L_iR^i\leq C_{\ell}$. 
% \end{definition}
% Then, using \citep{bach2017breaking}, Proposition 5 we can show that $(R, C_{\ell})$-smooth function is representable as follows.
% \begin{lemma}[Lemma A.5 in \citet{bai2024transformers}]
%     Suppose function $g:\bb R^d\to\bb R$ is $(R, C_{\ell})$ smooth. Then there exists a signed measure $\mu$ over $\ca V:=\{\bfa w\in\bb R^{d+1},\Vert\bfa w\Vert_2=1\}$ such that
%     \begin{align*}
%         g(\bfa x)=\int_{\ca V}\frac{}{}
%     \end{align*}
% \end{lemma}


\section{Omitted Proofs}
\begin{theorem}
    
\end{theorem}
\begin{proof}
We first consider the input matrix to be 
\begin{align*}
    \bfa H_1:=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_n\\
         \wha \mu_{1}^{(0)}&\wha \mu_{2}^{(0)}&\ldots&\bfa 0\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        &&\bfa 0&
    \end{bmatrix}\in\bb R^{D\times N}, 
\end{align*}
where $\wh z^{(0)}:[n]\to[k]$ is the assignment function, $\wha\mu_i\in\bb R^{d}$ is the initially estimated centroid for the $i$-th cluster. $\bfa p_{1,i}\in\bb R^k$ satisfies $\bfa p_{1,i,j}=\mbbm 1_{\wh z^{(0)}(i)=j}$ for all $j\in[k]$. And for $\bfa p_{2,i}$ we have $\bfa p_{2,i,j} = \mbbm 1_{j=i}$ for $i\leq d$ and $\bfa p_{2,i,j}=0$ for $i\leq N$ and $j\leq d$. We let $\bfa p_{3,1}=\bfa p_{3,2}=\ldots=\bfa p_{3,N} = \bfa 0\in\bb R^k$.
We note that algorithm \ref{alg:loyld} consists of two iterative steps: (1) The expectation step where we take the averages to get an initial estimate $\wha \mu_{\ell}^{(t)}$. (2) The maximization step where we assign each individual sample their labels. Our following discussions simulate the two steps separately as follows.
\begin{center}
    \textbf{1. The Expectation Step.}
\end{center}
For the expectation step, our network is designed by
\begin{align*}
    \bfa V^{(1)}_1&=\begin{bmatrix}
        \bfa 0_{d\times (D-d)}&\bfa 0\\
        I_d&\bfa 0\\
        \bfa 0&\bfa 0
    \end{bmatrix},\quad\bfa Q^{(1)}_1=\begin{bmatrix}
    \bfa 0_{k\times 2d}&I_k&\bfa 0\\       
        &\bfa 0&
    \end{bmatrix},\quad\bfa K^{(1)}_1=\begin{bmatrix}
        \bfa 0_{d\times(2d+k)}& I_{d}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\\
    \begin{bmatrix}
        \bfa 0_{d\times (D-d)}&\bfa 0\\
        I_d&\bfa 0\\
        \bfa 0&\bfa 0
    \end{bmatrix},\quad\bfa Q^{(1)}_1=\begin{bmatrix}
    \bfa 0_{k\times 2d}&I_k&\bfa 0\\       
        &\bfa 0&
    \end{bmatrix},\quad\bfa K^{(1)}_1=\begin{bmatrix}
        \bfa 0_{d\times(2d+k)}& I_{d}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\\
    \bfa V_2^{(1)} &= \begin{bmatrix}
        \bfa 0_{d\times d}&\bfa 0&\bfa 0\\
        \bfa 0_{d\times d}&-I_d &\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\quad\bfa Q_2^{(1)}=\bfa K_2^{(1)}=\begin{bmatrix}
        \bfa 0_{d\times d}&\bfa 0&\bfa 0\\
        \bfa 0_{d\times d}&-I_d &\bfa 0\\
        &\bfa 0&
    \end{bmatrix}.
\end{align*}
Then we can show that
\begin{align*}
    \bfa V_1^{(1)}\bfa H=\begin{bmatrix}
        &\bfa 0_{d\times N}&\\
        \bfa x_1&\ldots&\bfa x_N\\
        &\bfa 0&
    \end{bmatrix}, \quad\bfa Q_1^{(1)}\bfa H_1=\begin{bmatrix}
        (2\log n)\bfa p_{1,1}^{(0)}&\ldots&(2\log n)\bfa p_{1,N}^{(0)}\\
        &\bfa 0&
    \end{bmatrix},\quad\bfa K_1^{(1)}\bfa H_1=\begin{bmatrix}
        I_d&\bfa 0\\
        \bfa 0&\bfa 0
    \end{bmatrix}.
\end{align*}
Hence we can show that
\begin{align*}
   \softmax\Big( \lef(\bfa Q_1^{(1)}\bfa H_1\rig)^\top\lef(\bfa K_1^{(1)}\bfa H_1\rig)\Big)=\softmax\lef(\begin{bmatrix}
       C\log n\tda p_{1,1}^{(0),\top}&\bfa 0\\
       \vdots&\vdots\\
       C\log n\tda p_{1,N}^{(0),\top}&\bfa 0
   \end{bmatrix}\rig).
\end{align*}
We further note that
\begin{align*}
    \bigg|\frac{\exp(C\log N)}{\sum_{i=1}^N\mbbm 1_{\wh z_i^{(0)}=j}\exp(C\log N)+\mbbm 1_{\wh z_i^{(0)}\neq j}}-\frac{1}{\sum_{i=1}^N\mbbm 1_{\wh z_i^{(0)}=j}}\bigg|\leq N^{-C}.
\end{align*}
Similarly we have
\begin{align*}
    \bigg|\frac{1}{\sum_{i=1}^N\mbbm 1_{\wh z_i^{(0)}=j}\exp(C\log N)+\mbbm 1_{\wh z_i^{(0)}\neq j}}\bigg|\leq N^{-C}.
\end{align*}
And we can show that under this construction,
\begin{align*}
   \bfa V^{(5)}_1\bfa H_4 (\bfa Q^{(5)}_1\bfa H_4)^\top&=\begin{bmatrix}
       &&\bfa 0_{d}\\\wha\mu_1^{(1)}&\ldots&\wha\mu_k^{(1)}&\bfa 0\\
       &&\bfa 0&
   \end{bmatrix},\quad \bfa K^{(5)}\bfa H_4=\begin{bmatrix}
        I_d&\bfa 0\\
        \bfa 0&\bfa 0
    \end{bmatrix},\\
    \bfa V^{(5)}_2\bfa H_4(\bfa Q_2^{(5)}\bfa H_4)^\top(\bfa K_2^{(5)}\bfa H_4)&=\begin{bmatrix}
        &&\bfa 0_{d}&\\
        \wha\mu_1^{(0)}&\ldots&\wha\mu_k^{(0)}&\bfa 0\\
        &&\bfa 0&
    \end{bmatrix}
\end{align*}
And, we can show that
\begin{align*}
    \bfa H_{5,1} = \bfa H_4 +\bfa V^{(5)}\bfa H_4(\bfa Q^{(5)}\bfa H_4)^\top(\bfa K^{(5)}\bfa H_4)=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_{k}&\ldots&\bfa x_N\\
        \wha \mu_{1}^{(1)}&\wha \mu_{2}^{(1)}&\ldots&\wha \mu_{k}^{(1)}&\ldots&\bfa 0\\
        \bfa p^\prime_{1,1}&\bfa p^\prime_{1,2}&\ldots&\bfa p_{1,k}^\prime&\ldots&\bfa p^\prime_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,k}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1&\ldots&1\\
        &&\bfa 0&&&
    \end{bmatrix}.
\end{align*}
And the Expectation Step is concluded as we update the centroids from $\{\bfa\mu_i^{(0)}\}_{i\in[k]}$ to $\{\bfa\mu_i^{(1)}\}_{i\in[k]}$. The next step is to update the assignment $\bfa p_{1,i}^\prime$ to $\bfa p_{1,i}^{(1)}$ for $i\in[N]$.

\begin{center}
    \textbf{2. The Maximization Step.}
\end{center}
We further perform the expectation step by designing the following layers.
\begin{align*}
    \bfa V_i^{(4)}=\begin{bmatrix}
        &\bfa 0_{(3d+2k+1)\times D}&\\
        \bfa 0_{k\times2d}& I_k&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\quad\bfa Q_i^{(4)}=\begin{bmatrix}
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0_{k\times2d}& I_k&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix},\quad\bfa K_i^{(4)}=\begin{bmatrix}
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix}
\end{align*}
Then we further note that
\begin{align*}
    \bfa H_5 =\bfa H_4+\sum_{i=1}^2\bfa V_i^{(4)}\bfa H_4\softmax\lef(\rig)
\end{align*}
\end{proof}
% \begin{lemma}[Identity Mappings of the Softmax Function]
%     There exists a set of weights $((\bfa v_1, a_1),\ldots,(\bfa v_M,a_M))\in[\bb R^{d+1}\times[-B,B]]^M$. The mapping $f_i(\bfa x):=x_i$ can be approximated by a sum of the Softmax functions with the number of heads $M<$ such that
%     \begin{align*}
%         \sup_{0\leq\alpha\leq m}\Big|f(\bfa x)-\frac{1}{M}\Big|\leq\epsilon
%     \end{align*}
% \end{lemma}
% \begin{proof}
%     By lemma \ref{lm:a1} we can show that for $M\gtrsim C^2(d)B_f^2/\epsilon^2$ there exists $((\bfa v_1, a_1),\ldots,(\bfa v_M,a_M))\in[\bb R^{d+1}\times[-B,B]]^M$ such that the function $f(\bfa x)=x_i$ can be approximated with
%     \begin{align*}
%         \sup_{\bfa x\in U}\Big|f(\bfa x)-\frac{1}{M}\sum_{i=1}^Ma_i\sigmoid\lef([\bfa x^\top, 1]\bfa v_i\rig)\Big|\leq\epsilon.
%     \end{align*}
% \end{proof}
\begin{lemma}[Approximating the Hardmax Function by the Softmax Function] Consider a vector $\bfa x\in\bb R^d$. Let $x^*=\max_{i}\{x_i\}_{i\in[d]}$. Define $x^*=\max_{i\in[d]}x_i$, $\ca N_2=\{i:x_i=x^*\}$, $\Delta = x^*-\max_{i\in\ca N_2}x_i$. Define the Hardmax function as $\text{Hardmax}(\bfa x)=\begin{bmatrix}
    \frac{\mbbm 1_{x_1=\max_{i\in[d]}\{x_i\}}}{\sum_{i=1}^d\mbbm 1_{x_i=\max_{i\in[d]}}\{x_i\}}&\ldots&\frac{\mbbm 1_{x_d=\max_{i\in[d]}\{x_i\}}}{\sum_{i=1}^d\mbbm 1_{x_i=\max_{i\in[d]}}\{x_i\}}
\end{bmatrix}$, we subsequently show that 
\begin{align*}
    \Big|\softmax(\beta\bfa v)-\text{Hardmax}(\bfa v)\Big|\leq\bigg((d-|\ca N_2|)+\frac{(d-|\ca N_2|)^2}{|\ca N_2|^3}\bigg)^{\frac{1}{2}}\exp(-\beta\Delta).
\end{align*}
\end{lemma}
\begin{proof}
 We can show that the difference is given by
    \begin{align*}
        \Big\Vert\softmax(&\beta \bfa v)-\text{Hardmax}(\bfa v)\Big\Vert_{2} =\bigg(\sum_{i=1}^d\bigg(\frac{\mbbm 1_{x_i=\max_{i\in[d]}\{x_i\}}}{\sum_{i=1}^d\mbbm 1_{x_i=\max_{i\in[d]}\{x_i\}}}-\frac{\exp(\beta x_i)}{\sum_{i=1}^d\exp(\beta x_i)}\bigg)^2\bigg)^{\frac{1}{2}} \\
        &=\bigg(\sum_{i=1}^d\bigg(\frac{\mbbm 1_{x_i=\max_{i\in[d]}\{x_i\} }}{\sum_{i=1}^d\mbbm 1_{x_i=\max_{i\in[d]}\{x_i\} }}-\frac{\exp(\beta(x_i-x^*))}{\sum_{i=1}^d\exp(\beta(x_i-x^*)) }\bigg)\bigg)^{\frac{1}{2}}\\
        &\leq\bigg(\sum_{i=1}^d\mbbm 1_{x_i\neq x^*}\exp\lef(2\beta(x_i-x^*)\rig)+\mbbm 1_{x_i=x^*}\bl\frac{\exp\lef(\beta(x_i-x^*)\rig)}{\sum_{i=1}^d\exp\lef(\beta(x_i-x^*)
        \rig)}-\frac{1}{|\{i:x_i=x^*\}|}\br^2\bigg)^{\frac{1}{2}}\\
        &\leq \Big(|\ca N_1|\exp(-2\beta\Delta)+ |\ca N_2|\Big(\frac{1}{|\ca N_2|+|\ca N_1|\exp(-\beta \Delta)}-\frac{1}{|\ca N_2|}\Big)^2\Big)^{\frac{1}{
        2}}\\
        &\leq \bigg((d-|\ca N_2|)\exp(-2\beta\Delta) +\frac{(d-|\ca N_2|)^2\exp(-2\beta\Delta)}{|\ca N_2|\lef(|\ca N_2|+(d-|\ca N_2|)\exp(-\beta\Delta)\rig)^2}\bigg)^{\frac{1}{2}}\\
        &=\bigg((d-|\ca N_2|)+\frac{\lef(d-|\ca N_2|\rig)^2}{|\ca N_2|\lef(|\ca N_2|+(d-|\ca N_2|)\exp(-\beta\Delta)\rig)^2}\bigg)^{\frac{1}{2}}\exp\lef(-\beta\Delta\rig)\\
        &\leq \bigg((d-|\ca N_2|)+\frac{(d-|\ca N_2|)^2}{|\ca N_2|^3}\bigg)^{\frac{1}{2}}\exp(-\beta\Delta).
    \end{align*}
\end{proof}
\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
\cref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
\cref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\section{Additional Experiments}

\begin{figure}[htbp]
    \centering
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_dist_metrics_attn.pdf}
        % \subcaption{Top-10 Eigenvalues}
    \endminipage
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_min_dist_loss_attn.pdf}
        % \subcaption{RMSE with Varying Layers}
    \endminipage\vspace{-0.1em}
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_N_metrics_attn.pdf}
        % \subcaption{Cosine Similarity with Varying d}
    \endminipage
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_N_loss_attn.pdf}
        % \subcaption{Fourth Chart}
    \endminipage\vspace{-0.1em}
    \vspace{-1em}
    \caption{{\textbf{xxx.}
    We use a $3$-layer, $2$ head, $64$ hidden dimension Transformer to xxx}}
    % \label{fig:softmax_loss}
\end{figure}


\begin{figure}[htbp]
    \centering
\minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_num_classes_metrics_attn.pdf}
        % \subcaption{Top-10 Eigenvalues}
    \endminipage
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_num_classes_loss_attn.pdf}
        % \subcaption{RMSE with Varying Layers}
    \endminipage\vspace{-0.1em}
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_num_classes_metrics_attn.pdf}
        % \subcaption{Cosine Similarity with Varying d}
    \endminipage
    \minipage{0.45\textwidth}
        \includegraphics[width=\linewidth]{charts/multiclass/multiclass_synthetic_ratio_loss_attn.pdf}
        % \subcaption{Fourth Chart}
    \endminipage
    \vspace{-1em}
    \caption{{\textbf{Comparison of Concatenated Attention and Averaged Attention on the Real World Dataset.}
    \emph{Left: Performance Comparision on ARI and NMI.}
    \emph{Right: Performance Comparision on Converged Loss.}
    }
    }
    % \label{fig:softmax_loss}
\end{figure}




\end{document}


% This document was modified from the file originally made available by
% Pat Langley and Andrea Danyluk for ICML-2K. This version was created
% by Iain Murray in 2018, and modified by Alexandre Bouchard in
% 2019 and 2021 and by Csaba Szepesvari, Gang Niu and Sivan Sabato in 2022.
% Modified again in 2023 and 2024 by Sivan Sabato and Jonathan Scarlett.
% Previous contributors include Dan Roy, Lise Getoor and Tobias
% Scheffer, which was slightly modified from the 2010 version by
% Thorsten Joachims & Johannes Fuernkranz, slightly modified from the
% 2009 version by Kiri Wagstaff and Sam Roweis's 2008 version, which is
% slightly modified from Prasad Tadepalli's 2007 version which is a
% lightly changed version of the previous year's version by Andrew
% Moore, which was in turn edited from those of Kristian Kersting and
% Codrina Lauth. Alex Smola contributed to the algorithmic style files.


==> sections/sect4.tex <==
\section{Theoretical Results}\label{sect3}
This section presents our theoretical results and the idea of taking each step in the proof. Our proof constructs a particular instance of the transformers and shows that the forward propagation on our constructed instance approximates the Power Method. We also carefully design the contextual matrix $\bfa P$, explained as follows.

\paragraph{The Design of Auxillary Matrix.} Our design of the matrix $\bfa P$ consists of three parts:
\begin{enumerate}
    \item \emph{Place Holder.} For $\ell\in\{1\}\cup[4:k+3]$ and $i\in[N]$, we let $\tda p_{\ell, i}=\bfa 0\in\bb R^{d\times 1}$. The place holders in $\bfa P$ record the intermediate results in the forward propagation.
    \item \emph{Identity Matrix.} We let $ \begin{bmatrix}
        \tda p_{2,1}&\ldots&\tda p_{2,N}
    \end{bmatrix}=\begin{bmatrix}
        \bfa I_d&\bfa 0_{d\times(N-d)}
    \end{bmatrix}$. The identity matrix in $\bfa P$ helps us screen out all the covariates $\bfa X$ in the forward propagation.
    \item \emph{Random Samples on the Hypersphere.} We let $\tda p_{3,1},\ldots\tda p_{3,k}$ be the i.i.d. samples uniformly distributed on $\bb S^{d-1}$. The random samples on the sphere correspond to the initial vectors $\bfa v_{0,\ell}$ for $\ell\in[k]$ in algorithm \ref{alg:almoexactrecov}.
\end{enumerate}
Given the above construction on the auxiliary matrix $\bfa P$, we are ready to state the existence theorem in this work, given as follows.

\begin{algorithm}[htbp] 
 \caption{Spectral Clustering}
\label{alg:spectralclustering}
\KwData{$\bfa X\in\bb R^{D\times N}$ with $\bfa X_i\in\bb R^D$ for all $i\in[N]$}
 Compute the SVD of the data matrix $\bfa X=UDV^\top$. Let $U_k$ be the first $k$ columns of $U$\;

 Project $\bfa x_1,\ldots,\bfa x_N$ onto $U_k$, i.e. let $\wha x_i\gets U_kU_k^\top \bfa x_i$ \;
 Run an \emph{Transformer k-means++\cite{arthur2006k}} algorithm on the columns of projected matrix $\wha X=\begin{bmatrix}
     \wha x_1,\ldots,\wha x_N
 \end{bmatrix}$\;
\end{algorithm}
\begin{assumption}\label{asumpt1}
    We assume that $\bfa X_1,\ldots,\bfa X_N$ are i.i.d. samples from $\sum_{\ell=1}^k\pi_\ell\bb P(X|\mu)$. Minimal separation is denoted by $\Delta:=\inf_{i\neq j}\Vert\bfa\mu_i-\bfa\mu_j\Vert_2$.
\end{assumption}

And the kmeans++ algorithm is given by the following procedure.
\begin{algorithm}[htbp] 
 \caption{k-means++}
\label{alg:kmeans++}
\KwData{$\bfa X\in\bb R^{k\times N}$ with $\bfa X_i\in\bb R^k$ for all $i\in[N]$}
Choose an initial center $\bfa c_1$ uniformly at random from $\ca X:=\{\bfa X_1,\ldots,\bfa X_N\}$ and let $\ca C=\{\bfa c_1\}$\;
\While{$|\ca C|<k$}{Choose the next center $\bfa c$, selecting $\bfa c=\bfa x\in\ca X$ with probability $\frac{D(\bfa x)}{\sum_{x\in\ca X}D(\bfa x)}$\\
where $D(\bfa x):=\argmin_{\bfa c\in\ca C}\Vert \bfa c-\bfa x\Vert_2$\;
If $\bfa c\notin\ca C$, let $\ca C\gets\ca C\cup\{\bfa c\}$\;
}
Run the Lloyd's algorithm with covariates $\bfa X$ and initial centroids $\ca C$\;
\end{algorithm}
\begin{algorithm}[htbp] 
 \caption{Lloyd's Algorithm}
\label{alg:lloyd}
\KwData{$\bfa X\in\bb R^{k\times N}$ and initial clusters $\ca C=\lef\{\wha\mu_\ell^{(0)}\rig\}_{\ell\in[k]}$}
Let $t\gets 1$\;
Initialize with the starting membership $\wh z_i^{(0)}\gets\argmin_{\ell\in[k]}\Vert \bfa x_i-\wha\mu_\ell^{(0)}\Vert_{\Sigma^{-1}}$\;
\While{$\exists j\in[n]$ such that $\wh z^{(t+1)}_j\neq \wh z^{(t)}_j$}{Update the centroids and memberships through $\wha\mu_{\ell}^{(t)}\gets\frac{\sum_{i=1}^n\bfa x_{i}\mbbm 1_{\wh z_i^{(t-1)}=\ell}}{\sum_{i=1}^n\mbbm 1_{\wh z_i^{(t-1)}=\ell}},\enspace\forall \ell\in[k],\qquad \wh z_i^{(t)}\gets\argmin_{\ell\in[k]}\Vert \bfa x_i-\wha\mu_{\ell}^{(t)}\Vert^2_{\Sigma^{-1}},\enspace\forall i\in[n].$
}
Run the Lloyd's algorithm with $\bfa X$ and $\ca C$\;
\end{algorithm}

In particular, take as input the context given by $\bfa H=\begin{bmatrix}
    \bfa x_1,\ldots,\bfa x_N\\
    \bfa p_1,\ldots,\bfa p_N
\end{bmatrix}\in\bb R^{D\times N}$, we show that the Transformer network can approximate the spectral clustering algorithm in the initialization phase, given by \ref{alg:spectralclustering}.
\subsection{The Power Iteration Method}
In the first step of the power method 
we use the Transformer model to approximate the singular vectors of the matrix $\bfa X^\top\bfa X$. A typical implementation to achieve this is given by the power method.


\begin{theorem}[Transformer Approximation of the Power Iteration]\label{thm3.1} Denote the eigenvalues of $\bfa X\bfa X^\top$ to be $\lambda_1>\lambda_2>\ldots>\lambda_k>\ldots$. Let $\Delta:=\min_{1\leq i<j\leq k}|\lambda_i-\lambda_j|$. Assume that the eigenvalues of $\bfa X$ satisfy $\Vert\bfa X\Vert_2\leq B_X$. Assume that the initialized vectors $\tda p_{3,1},\ldots\tda p_{3,N}$ 
    satisfy  $\tda p_{3,i}^\top\bfa v_{i}\geq\delta$ for all $i\in[k]$ and make the rest of the vectors $\bfa 0$. 
    Then, there exists a transformer model with number of layers $L=2\tau+4k+1$ and number of heads $M\leq \lambda_1^d\frac{C}{\epsilon^2}$ with $\tau\leq\frac{\log(1/\epsilon_0\delta)}{\epsilon_0}$ such that for all $\epsilon_0,\epsilon>0$,
    the final output $\wha v_1,\ldots,\wha v_{k}$ given by the transformer model achieve
    \begin{align*}
        \lef\Vert\wha v_{\eta+1}-\bfa v_{\eta+1}\rig\Vert_2\leq C\tau \epsilon\lambda_1^2+\frac{C\lambda_1\sqrt{\epsilon_0}}{\Delta}\prod_{i=1}^{\eta}\frac{5\lambda_{i+1}}{\Delta}.
    \end{align*} 
    Moreover, consider the accuracy of multiple $\bfa v$s as a whole. There exists $\bfa\theta$ such that 
    \begin{align*}
        L\lef(TF_{\wha\theta}(\bfa H),\bfa V\rig)\leq C\tau\epsilon k\lambda_1^2+C\bl\frac{\epsilon_0\lambda_1^2}{\Delta^2}\sum_{\eta=1}^{k-1}\prod_{i=1}^{\eta}\frac{25\lambda_{i+1}^2}{\Delta^2}\br^{1/2}.
    \end{align*}
\end{theorem}
\begin{remark}
\label{remark3}
    The approximation error consists of two terms. The first term comes from the approximation of the Power Method iterations by transformers. The second term comes from the error caused by finite iteration $\tau$. To acquire a more direct account of the error terms and its order of magnitude, we consider a special case where the eigenvalues $\lambda_1\asymp\lambda_2\asymp\ldots\asymp\lambda_k\asymp\Delta$. Then our results boil down to 
    \begin{align*}
        \lef\Vert TF_{\bfa\theta}(\bfa H)-\begin{bmatrix}
            \bfa v_1^\top,\bfa v_2^\top,\ldots,\bfa v_k^\top
        \end{bmatrix}^\top\rig\Vert_2\leq C\tau\epsilon k \lambda_1^2+ C\frac{\lambda_1}{\Delta}\sqrt{k\epsilon_0}.
    \end{align*}
    These results hide dimension $d$ in the universal constant. Hence the dimension significantly affects the approximation properties of transformers. Our experimental results in section \ref{sect4} also indicate that learning high dimensional principal eigenvectors is challenging.
\end{remark}
We show that the conditions on $\tda p_{3,1},\ldots,\tda p_{3,N}$ can be achieved through sampling from isotropic Gaussians, given by the following lemma.
    \begin{lemma}\label{lm3.1.1}\label{lm3.1}
        Let $\bfa y\in\bb R^d$ be a random vector with isotropic Gaussian as its probability density. Consider $\bfa x=\frac{\bfa y}{\Vert\bfa y\Vert_2}$. Let $\bfa v$ be any unit length vector, then we have for all $\delta<\frac{1}{2}d^{-1}$,
           $ \bb P\lef(|\bfa v^\top\bfa x|\leq\delta\rig)\leq  \frac{1}{\sqrt{\pi}}\sqrt\delta+\exp\lef(-C\delta^{-\frac{1}{2}}\rig)$.
        Therefore, for all $\delta<\frac{1}{2}d^{-1}$, the event in theorem \ref{thm3.1} is achieved with
        \begin{align*}
             \bb P\bl\exists i\in[k]\text{ such that }&\bfa x_i^\top\bfa v_i\leq\frac{\delta}{\sqrt d}\br\leq \frac{k\sqrt{\delta}}{\sqrt{\pi}}+k\exp(-C\delta^{-1}).
        \end{align*}
    \end{lemma}
Given the approximation error provided by theorem \ref{thm3.1}, we further provide the generalization error bound for the ERM defined by \eqref{ERM}. This requires us to consider the following regularity conditions on the underlying distribution of $\bfa X\bfa X^\top$ (which also translates to the distribution of $\bfa X$).
\begin{assumption}\label{assump1}
    The distribution of $\bfa X\bfa X^\top$ supports on $$\bb X:=\lef\{A:A\in\bfa S^d_{++},  B_X\geq\lambda_1(A)>\lambda_2(A)>\ldots>\lambda_k(A),\inf_{1\leq i<j\leq k}\lambda_i(A)-\lambda_j(A)\geq\Delta\rig\}.$$
\end{assumption}
\begin{remark}
    The above assumption can be easily generalized to distribution that supports on $\bb X$ with high probability. Examples of such distribution include the Wishart distribution under the Gaussian design. In this work, we stick to the simplest case where the maximum eigenvalue is bounded from above.
\end{remark}
Given the above assumption, we are ready to state the generalization bound.
\begin{proposition}\label{genbound}
   With probability at least $1-\xi$, the ERM solution $\wha\theta$ satisfies
    \begin{align*}
        \bb E\lef[L\lef(TF_{\wha\theta}(\bfa H),\bfa V\rig)|\wha\theta\rig]&\leq\inf_{\bfa\theta\in\Theta(B_{\bfa\theta},B_M)}\bb E\lef[L\lef(TF_{\bfa\theta}(\bfa H),\bfa V\rig)\rig]\\
        &+ C \sqrt{\frac{k^3LB_Md^2\log(B_{\theta}+B_X+k)+\log(1/\xi)}{n}}.
    \end{align*}
\end{proposition}
   Together with the bound given by theorem \ref{thm3.1} and lemma \ref{lm3.1.1}, which essentially give a high probability upper bound on $\inf_{\bfa\theta\in\Theta(B_{\bfa\theta},B_M)}$ we can derive a general upper bound on the generalization error, given as follows.
    \begin{corollary}
        Under assumption \ref{assump1}, with probability at least $1-\xi-\frac{k\sqrt\delta}{\sqrt\pi}-k\exp\lef(-C\delta^{-1/2}\rig)$ for all $\delta<d^{-1}$ we have for all $\epsilon,\epsilon_0>0$,
        \begin{align*}
            \bb E\lef[L\lef(TF_{\wha\theta}(\bfa H),\bfa V\rig)|\wha\theta\rig]&\leq \bb E\lef[C\tau\epsilon k\lambda_1^2+C\bl\frac{\epsilon_0\lambda_1^2}{\Delta^2}\sum_{\eta=1}^{k-1}\prod_{i=1}^{\eta}\frac{25\lambda_{i+1}^2}{\Delta^2}\br^{1/2}\rig]\\
            &+C\sqrt{\frac{k^3\log(\delta/
            \epsilon_0)\lambda_1^d d^2\log(B_{\theta}+B_X+k)+\log(1/\xi)}{n\epsilon_0\epsilon^2}}.
        \end{align*}
    \end{corollary}
    \begin{remark}
        If we consider optimizing the bound w.r.t. $\epsilon_0$ and $\epsilon$, we obtain that $\bb E\lef[L(TF_{\wha\theta}(\bfa H),\bfa V)|\wha\theta\rig]\lesssim n^{-1/5}$ given that the rest of the parameters are of constant scales. It is not known if the results are improvable or not and the authors believe this question worth future explorations.
    \end{remark}
The next theorem demonstrates that there exists a Transformer that simulates the expectation maximization algorithm on Gaussian mixture model.
\begin{theorem}
    
\end{theorem}
\begin{proof}
We first consider the input matrix to be 
\begin{align*}
    \bfa H_1:=\bfa H=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_n\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(n)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa p_{3,1}&\bfa p_{3,2}&\ldots&\bfa p_{3,N}
    \end{bmatrix}\in\bb R^{D\times N}, 
\end{align*}
where $\wh z^{(0)}:[n]\to[k]$ is the assignment function, $\wha\mu_i\in\bb R^{d}$ is the initially estimated centroid for the $i$-th cluster. $\bfa p_{1,i}\in\bb R^k$ satisfies $\bfa p_{1,i,j}=\mbbm 1_{\wh z^{(0)}(i)=j}$ for all $j\in[k]$. And for $\bfa p_{2,i}$ we have $\bfa p_{2,i,j} = \mbbm 1_{j=i}$ for $i\leq d$ and $\bfa p_{2,i,j}=0$ for $i\leq N$ and $j\leq d$. We let $\bfa p_{3,1}=\bfa p_{3,2}=\ldots=\bfa p_{3,N} = \bfa 0\in\bb R^k$.
We note that algorithm \ref{alg:lloyd} consists of two iterative steps: (1) The expectation step where we take the averages to get an initial estimate $\wha \mu_{\ell}^{(t)}$. (2) The maximization step where we assign each individual their labels. Our following discussions treat the two steps separately. 
\begin{center}
    \textbf{1. The Expectation Step.}
\end{center}
To achieve the first step, we construct our transformer weights as follows:
\begin{align*}
    \bfa V_1^{(1)}=\begin{bmatrix}
        \tda V_{1,1}^{(1)}&\tda V_{1,2}^{(1)}&\tda V_{1,3}^{(1)}
    \end{bmatrix},\quad\bfa Q_1^{(1)}=\begin{bmatrix}
        \bfa 0_{1\times(3d+k)}&1&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix},\quad\bfa K_1^{(1)}=\begin{bmatrix}
        \bfa 0_{1\times(3d+k)}&1&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix},
\end{align*}
where $\tda V_{1,1}^{(1)}\in\bb R^{2d\times D}=\bfa 0$, $\tda V_{1,2}^{(1)}=\begin{bmatrix}
        \bfa 0_{3d+k}\\
        I_k\\
        \bfa 0
    \end{bmatrix}\in\bb R^{k\times D}$. Then we can show that
\begin{align*}
   (\bfa K_1^{(1)}\bfa H_1)^\top=(\bfa Q_1^{(1)}\bfa H)^\top = \begin{bmatrix}
        1&\bfa 0\\
        \vdots &\bfa 0\\
        1&\bfa 0
    \end{bmatrix}.
\end{align*}
Then we can show that
\begin{align*}
   (\bfa Q_1^{(1)}\bfa H)^\top(\bfa K_1^{(1)}\bfa H) = \begin{bmatrix}
       \bfa v_1&\ldots&\bfa v_1
   \end{bmatrix},\quad \bfa v_{1,i} = 1\quad\forall i\in[N].
\end{align*}
Hence, we can obtain that
\begin{align*}
    \bfa V_1^{(1)}\bfa H&\times\sigma((\bfa Q_1^{(1)}\bfa H)^\top(\bfa K_1^{(1)}\bfa H))=\bfa V_1\bfa H\times\begin{bmatrix}
        \bfa v_1 &\ldots&\bfa v_1
    \end{bmatrix}=\bfa V_1\times \begin{bmatrix}
        &\bfa A_0&\\
        \bfa v_k &\ldots&\bfa v_k\\
        &\bfa A_1&
    \end{bmatrix}\\
    &=\begin{bmatrix}
        \tda V_{1,1}^{(1)}&\tda V_{1,2}^{(1)}&\tda V_{1,3}^{(1)}
    \end{bmatrix}\begin{bmatrix}
        &\bfa A_0&\\
        \bfa v_k&\ldots&\bfa v_k\\
        &\bfa A_1&
    \end{bmatrix}=\tda V_{1,2}^{(1)}\begin{bmatrix}
        \bfa v_k &\ldots&\bfa v_k
    \end{bmatrix}\\
    &=\begin{bmatrix}
        \bfa 0_{3d+k}\\
        I_k\\
        \bfa 0
    \end{bmatrix}\begin{bmatrix}
        \bfa v_k&\ldots&\bfa v_k
    \end{bmatrix}=\begin{bmatrix}
        &\bfa 0_{3d+k}&\\
        \bfa v_k&\ldots&\bfa v_k\\
        &\bfa 0&
    \end{bmatrix},
\end{align*}
 where $\bfa A_0\in\bb R^{2d\times N}$ and $
    \bfa v_{k,\ell}=\sum_{i=1}^N\mbbm 1_{\wh z_i^{(0)}=\ell}$.
Then it is checked that
\begin{align*}
   \bfa H_2 =  \bfa H_1+ \bfa V_1^{(1)}\bfa H_1\times\sigma\lef((\bfa Q_1^{(1)}\bfa H_1)^\top(\bfa K_1^{(1)}\bfa H_1)\rig)=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa v_k&\bfa v_k&\ldots&\bfa v_k\\
        \bfa p_{4,1}& \bfa p_{4,2}&\ldots &\bfa p_{4,N}
    \end{bmatrix}.
\end{align*}
Therefore, we further construct the following multi-head layer to remove the off-diagonal elements in $\begin{bmatrix}
    \bfa v_k&\bfa v_k&\ldots&\bfa v_k
\end{bmatrix}$, given by 
\begin{align*}
    \bfa V_i^{(2)} = \begin{bmatrix}
        &\bfa 0_{(3d+2k+i)\times D}&\\
        \bfa 0_{1\times(3d+2k+i)}&1&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\quad \bfa Q_1^{(2)} = \begin{bmatrix}
        b
    \end{bmatrix},\quad\bfa K_1^{(2)} = \begin{bmatrix}
        c
    \end{bmatrix},\qquad\text{ for }i\in[k].
\end{align*}
Given this formulation, we can show that
\begin{align*}
    \sigma((\bfa Q_i^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2)) = \begin{bmatrix}
        &\bfa 0_{(i-1)\times N}&\\
        \bfa 0_{1\times(i-1)}&1&\bfa 0\\
        &\bfa 0&
    \end{bmatrix}.
\end{align*}
Hence, we can further show that
\begin{align*}
    \bfa V_{i}^{(2)}\bfa H_2\sigma((\bfa Q_i^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2))=\begin{bmatrix}
        &\bfa 0_{(3d+2k+i)\times D}&\\
        \bfa 0_{(i-1)}&\bfa v_{k,i}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},
\end{align*}
which immediately implies that
\begin{align*}
    \sum_{i=1}^k\bfa V_i^{(2)}\bfa H_2\sigma\lef((\bfa Q_i^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2)\rig)=\begin{bmatrix}
        \bfa 0_{(3d+2k)\times N}&\\
        \diag(\bfa v_k)&\bfa 0\\
        \bfa 0
    \end{bmatrix}.
\end{align*}
Given the above design, we can show that
\begin{align*}
    \bfa H_{3,1}=\bfa H_2+\sum_{i=1}^k\bfa V_i^{(2)}\bfa H_2\sigma\lef((\bfa Q_i^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2)\rig)=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa v_k&\bfa v_k&\ldots&\bfa v_k\\
        \diag(\bfa v_k)&&\bfa 0&\\
        &\bfa 0&&
    \end{bmatrix}.
\end{align*}
Then, we construct the MLP layer to remove the $\bfa v_k$ part, which is designed by
\begin{align*}
    \bfa W_1^{(2)}=I_D,\quad \bfa W_2^{(2)}= \begin{bmatrix}
        &\bfa 0_{(3d+k)\times D}&&\\
        \bfa 0_{k\times (3d+k)}&-I_k&I_k&\bfa 0_{}\\
       \bfa 0 &-I_k&\bfa 0&\bfa 0\\
       &\bfa 0&&
    \end{bmatrix}.
\end{align*}
Given this formulation, we can show that
\begin{align*}
    \bfa H_3 := \bfa H_{3,1}+\bfa W_1^{(2)}\sigma\lef(\bfa W_2^{(2)}\bfa H_{3,1}\rig)=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa v_k&\bfa v_k&\ldots&\bfa v_k\\
        \diag(\bfa v_k)&&\bfa 0&\\
        &\bfa 0&&
    \end{bmatrix}.
\end{align*}

% Then we consider the following attention head which essentially remove the $\bfa v_k$ part in $\bfa H_2$. We note that the rank of $\sigma((\bfa Q_i\bfa H_2)^\top(\bfa K_i\bfa H_2))$ is at most $D$. To form the 
% \begin{align*}
%     \bfa V_{k+1}^{(2)} = \begin{bmatrix}
%         &\bfa 0_{(3d+k)\times D}&\\
%         \bfa 0_{k\times (3d+k)}&-I_k&\bfa 0_{}\\
%         &\bfa 0&
%     \end{bmatrix},\quad \bfa Q_{k+1}^{(2)}=,\quad \bfa K_{k+1}^{(2)}=
% \end{align*}
% Given the above design, we can show that
% \begin{align*}
%     \bfa V_{k+1}^{(2)}\bfa H_2\sigma\lef((\bfa Q_{k+1}^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2)\rig)=\begin{bmatrix}
%         &\bfa 0_{(3d+k)\times N}&\\
%         -\bfa v_k&\ldots&-\bfa v_k\\
%         &\bfa 0&
%     \end{bmatrix}.
% \end{align*}
% Therefore, collecting pieces, we can show that
% \begin{align*}
%    \bfa H_3:= \bfa H_2 + \sum_{i=1}^{k+1}\bfa V_i^{(2)}\bfa H_2\sigma\lef((\bfa Q_i^{(2)}\bfa H_2)^\top(\bfa K_i^{(2)}\bfa H_2)\rig)=\begin{bmatrix}
%         \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
%         \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
%         \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
%         \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
%         1&1&\ldots&1\\
%         \diag(\bfa v_k)&&\bfa 0&\\
%         \bfa p_{4,1}& \bfa p_{4,2}&\ldots &\bfa p_{4,N}
%     \end{bmatrix}.
% \end{align*}
The following layer converts the term $\diag(\bfa v_k)$ to $\diag(\bfa v_k^\prime)$ where $\bfa v_{k,i}^\prime = 1/\bfa v_{k,i}$. The design is given as follows
\begin{align*}
    \bfa V_{i}^{(3)} &= \begin{bmatrix}
        &\bfa 0_{(3d+3k+1)\times D}&\\
        \bfa 0_{k\times(2d+2k)}&\diag(c_i)_{k\times k}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\quad\bfa Q_{i}^{(3)}=\begin{bmatrix}
        &\bfa 0_{(3d+3k+1)\times D}&\\
        \bfa 0_{k\times(2d+2k)} &I_{k}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\\
    \bfa K_{i}^{(3)}&=\begin{bmatrix}
        &\bfa 0_{(3d+3k+1)\times D}&\\
        \bfa 0_{k \times (3d+3k+1)}&\diag(a_i)_{k\times k}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix}\begin{bmatrix}
        &\bfa 0_{(3d+3k+1)\times D}&\\
       \bfa 0_{k\times(3d+2k+1)}&I_{k} &\bfa 0\\
       &\bfa 0&
    \end{bmatrix},
\end{align*}
where we show in lemma \ref{reluapprox} that for $M>\frac{1}{\epsilon^2}\log(1+C/\epsilon)$, there exists $\{a_i\}_{i\in[M]}$ such that for $x>1$, we have 
\begin{align*}
    \bigg\Vert\sum_{i=1}^Mc_i\sigma(a_ix) - \frac{1}{x}\bigg\Vert_2\leq\epsilon.
\end{align*}
And when $x=0$, we automatically obtain that 
$   \sum_{i=1}^Mc_i\sigma(0) =0$. We then immediately obtain that
\begin{align*}
    \bfa H_{4,1}:&=\bfa H_3 + \sum_{i=1}^M\bfa V_i^{(3)}\sigma\lef((\bfa Q_i^{(3)}\bfa H_3)^\top(\bfa K_i^{(3)}\bfa H_3)\rig)= \begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa v_k&\bfa v_k&\ldots&\bfa v_k\\
        \diag(\bfa v_k)&&\bfa 0&\\
        \diag(\bfa v_k^\prime)&&\bfa 0&\\
        &\bfa 0&&
    \end{bmatrix}+O_{2}(\epsilon),
\end{align*}
where $\bfa v_{k,i}^\prime = \bfa v_{k,i}^{-1}$. Then we apply the MLP again with the following design 
\begin{align*}
    \bfa W_1^{(4)}= I_D,\quad\bfa W_2^{(4)}=\begin{bmatrix}
        &\bfa 0_{(3d+k)\times D}&&\\
        \bfa 0_{k\times(3d+k)}&-I_k&I_k&\bfa 0\\
        \bfa 0&-I_k&\bfa 0&\bfa 0\\
        &\bfa 0&&
    \end{bmatrix}.
\end{align*}
The above construction implies that
\begin{align*}
    \bfa H_4 =\bfa W_2^{(3)}\sigma\lef(\bfa W_1^{(3)}\bfa H_3\rig) = \begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \bfa v_k&\bfa v_k&\ldots&\bfa v_k\\
        \diag(\bfa v_k^\prime)&&\bfa 0&\\
        &\bfa 0&&
    \end{bmatrix}.
\end{align*}
We construct the following layer to perform the normalization, given by 
\begin{align*}
    \bfa V_2^{(4)}&=-\bfa V_{1}^{(4)}= \begin{bmatrix}
    &\bfa 0_{(3d+2k+1)\times D}& \\
    \bfa 0_{k\times(3d+k+1)}&I_{k}&\bfa 0\\
    &\bfa 0&
    \end{bmatrix},\quad \bfa Q_1^{(4)} =-\bfa Q_2^{(4)}= \begin{bmatrix}
        &\bfa 0_{(3d+2k+1)\times D}&\\
        \bfa 0_{k\times 3d}&I_{k}&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\\
    \bfa K_1^{(4)}&=\bfa K_2^{(4)}=\begin{bmatrix}
        &\bfa 0_{(3d+2k+1)\times D}&\\
        \bfa 0_{k\times (3d+1)}&I_k&\bfa 0\\
        &\bfa 0&
    \end{bmatrix}.
\end{align*}
Then we can show that
\begin{align*}
    \sigma\lef((\bfa Q_1^{(4)}\bfa H_4)^\top(\bfa K_1^{(4)}\bfa H_4)\rig)-\sigma\lef((\bfa Q_2^{(4)}\bfa H_4)^\top(\bfa K_2^{(4)}\bfa H_4)\rig) = \begin{bmatrix}
        &\bfa 0_{(3d+2k+1)\times D}&\\
        \bfa p_{1,1}&\ldots&\bfa p_{1,N}\\
        &\bfa 0
    \end{bmatrix}.
\end{align*}
And we also have
\begin{align*}
    \bfa V_2^{(4)}\bfa H_4 = \begin{bmatrix}
        &\bfa 0_{(3d+3k+1)\times D}&\\
        \bfa 0_{k\times(3d+2k+1)}&\diag(\bfa v_k^\prime) &\bfa 0\\
        &\bfa 0&
\end{bmatrix}+O_2(\epsilon),
\end{align*}
which implies that
\begin{align*}
    \bfa H_{4,1} = \bfa H_3+\sum_{i=1}^2\bfa V_i^{(4)}\bfa H_3\times\sigma\lef((\bfa Q_i^{(4)}\bfa H_3)^\top(\bfa K_i^{(3)}\bfa H_3)\rig)=\begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p_{1,1}&\bfa p_{1,2}&\ldots&\bfa p_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \diag(\bfa v_k^\prime)&&\bfa 0&\\
        \bfa p_{1,1}^\prime&\bfa p_{1,2}^\prime&\ldots&\bfa p_{1,N}^\prime
    \end{bmatrix}+O_{2}(\epsilon),
\end{align*}
where $\bfa p_{1,i}^\prime = \diag(\bfa v_k^\prime)\bfa p_{1,i}$ for all $i\in[N]$. We therefore construct an MLP layer to replace the $\bfa p_{1}$ part using the following design
\begin{align*}
    \bfa W_1^{(4)}=I_D,\qquad\bfa W_2^{(4)} = \begin{bmatrix}
        &\bfa 0_{2d\times D}&&\\
        \bfa 0_{k\times 2d}&-I_k&\bfa 0&I_k&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0&\bfa 0&\bfa 0\\
        \bfa 0_{k\times 2d}&-I_k&\bfa 0&\bfa 0 &\bfa 0\\
    \end{bmatrix},
\end{align*}
which ultimately leads to 
\begin{align*}
    \bfa H_4 = \bfa W_1^{(3)}\sigma\lef(\bfa W_2^{(3)}\bfa H_3\rig) = \begin{bmatrix}
        \bfa x_1&\bfa x_2&\ldots&\bfa x_N\\
        \wha \mu_{\wh z^{(0)}(1)}^{(0)}&\wha \mu_{\wh z^{(0)}(2)}^{(0)}&\ldots&\wha \mu_{\wh z^{(0)}(N)}^{(0)}\\
        \bfa p^\prime_{1,1}&\bfa p^\prime_{1,2}&\ldots&\bfa p^\prime_{1,N}\\
        \bfa p_{2,1}&\bfa p_{2,2}&\ldots&\bfa p_{2,N}\\
        1&1&\ldots&1\\
        \diag(\bfa v_k^\prime)&&\bfa 0&\\
        &\bfa 0&&
    \end{bmatrix}.
\end{align*}
We can further perform the expectation step by the following layer
\begin{align*}
    \bfa V_i^{(4)}=\begin{bmatrix}
        &\bfa 0_{(3d+2k+1)\times D}&\\
        \bfa 0_{k\times2d}& I_k&\bfa 0\\
        &\bfa 0&
    \end{bmatrix},\quad\bfa Q_i^{(4)}=\begin{bmatrix}
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0_{k\times2d}& I_k&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix},\quad\bfa K_i^{(4)}=\begin{bmatrix}
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0\\
        \bfa 0&\bfa 0&\bfa 0
    \end{bmatrix}
\end{align*}
Then it is further noted that
\begin{align*}
    \bfa H_5 =\bfa H_4+\sum_{i=1}^2\bfa V_i^{(4)}
\end{align*}
\end{proof}
% The rest of this section presents a proof sketch on theorem \ref{thm3.1}.
% \paragraph{Proof Sketch of Theorem \ref{thm3.1}.}
%     The proof sketch for theorem \ref{thm3.1} goes by two important steps:



%     To obtain $\tda p_{3,i}$ for $i\in[k]$, we generate through the probablistic method, which gives the following lemma.
%     % \begin{lemma}
%     %     Let $\bfa y\in\bb R^d$ be a random vector with isotropic Gaussian as its probability density. Consider $\bfa x=\frac{\bfa y}{\Vert\bfa y\Vert_2}$. Let $\bfa v$ be any unit length vector, then we have
%     %        $$ \bb P\bl|\bfa v^\top\bfa x|\leq\frac{\epsilon}{\sqrt d}\br\leq  \frac{1}{\sqrt{\pi}}\epsilon+\exp\lef(-Cd\rig).$$
%     %     Therefore, the event in theorem \ref{thm3.1} can be estimated as
%     %     \begin{align*}
%     %          \bb P\bl\exists i\text{ such that }&\bfa x_i^\top\bfa v_i\leq\frac{\epsilon}{\sqrt d}\br\leq 1-\bl1-\frac{\epsilon}{\sqrt{\pi}}-\exp(-Cd)\br^k\leq \frac{k\epsilon}{\sqrt{\pi}}+k\exp(-Cd).
%     %     \end{align*}
%     % \end{lemma}

%     % \begin{align*}
%     %    \Bigg\Vert \tda H^{rpe,2}-\begin{bmatrix}
%     %         \bfa X\\
%     %         \tda y\\
%     %         \bfa X\bfa X^\top,\bfa 0\\
%     %         \tda p_{2,1},\ldots,\tda p_{2,N}\\
%     %         \tda p_{3,1},\ldots,\tda p_{3,N}\\
%     %         \tda p_{3,1}^{(\tau)},\bfa 0\\
%     %         \Vert\bfa X\bfa X^\top\tda p_{3,N}^{(\tau)}\Vert_2,\bfa 0
%     %     \end{bmatrix}\Bigg\Vert_2\leq\epsilon \Vert\bfa X\bfa X^\top\tda p_{3,1}\Vert_2.
%     % \end{align*}
%     % Then we can show that
%     % \begin{align*}
%     %     &\Bigg\Vert\bfa K\tda H^{pow,2\tau+2}-\begin{bmatrix}
%     %         \bfa 0_{(5d+1)\times(4d+1)}&\bfa 0_{(5d+1)\times 1}&\bfa 0\\
%     %         \bfa 0_{d\times(4d+1)}&\tda p_{3,1}^{(\tau)}&\bfa 0\\
%     %         \bfa 0&\bfa 0&\bfa 0
%     %     \end{bmatrix}\Bigg\Vert_2\leq \tau\epsilon\Vert\bfa X\bfa X^\top\Vert_2,\\ 
%     %     &\Bigg\Vert\bfa Q\tda H^{pow,2\tau+2}-\begin{bmatrix}
%     %         \bfa 0_{(5d+1)\times 1}&\bfa 0\\
%     %        \Vert\bfa X\bfa X^\top\tda p_{3,1}^{(\tau)}\Vert_2 \tda p_{3,1}^{(\tau)}&\bfa 0\\
%     %         \bfa 0&\bfa 0
%     %     \end{bmatrix}\Bigg\Vert_2\leq\tau\epsilon\Vert\bfa X\bfa X^\top\Vert_2.
%     % \end{align*}
%     % which immediately implies that
%     % \begin{align*}
%     %     \Bigg\Vert(\bfa K\tda H^{pow,2\tau+2})^\top(\bfa Q\tda H^{pow,2\tau+2})-\begin{bmatrix}
%     %         \bfa 0&\bfa 0\\
%     %         \Vert\bfa X\bfa X^\top\tda p_{3,1}\Vert_2\tda p_{3,1}^{(\tau)}\tda p_{3,1}^{(\tau),\top}&\bfa 0\\
%     %         \bfa 0&\bfa 0
%     %     \end{bmatrix}\Bigg\Vert_2
%     % \end{align*}
% \begin{lemma}\label{lm3.2}
% Assume that the correlation matrix $\bfa X\bfa X^\top$ has eigenvalues $\lambda_1>\lambda_2>\ldots>\lambda_{k}$. Assume that the eigenvectors are given by $\bfa v_1,\bfa v_2,\ldots,\bfa v_n$ and the eigenvalues satisfy $\inf_{i\neq j}|\lambda_i-\lambda_j|=\Delta$. Then, given that the estimate for the first $\tau$ eigenvectors satisfy
% $    \bfa v_i^\top\wha v_i\geq 1-\epsilon_i $ and the eigenvalues satisfy $|\lambda_i-\wh\lambda_i|\leq\delta_i$, the principle eigenvector of $\bfa X\bfa X^\top-\sum_{i=1}^{\tau}\wh\lambda_i\wha v_i\wha v_i^\top$ denoted by $\tda v_{\tau+1}$ satisfies
% \begin{align*}
%     \Vert\tda v_{\tau+1}-\bfa v_{\tau+1}\Vert_2 \leq\frac{\max_{i\in[\tau]}\delta_i+\sum_{i=1}^\tau\sqrt8\lambda_i\sqrt{\epsilon_i}}{\Delta}.
% \end{align*}
% Alternatively, we can also show that the eigenvector $\wha v_{\tau+1}$ returned by power method with $k= \frac{\log(1/\epsilon_0\delta)}{2\epsilon_0}$ that is initialized by  satisfies
% \begin{align*}
%     \wha v_{\tau+1}^\top\bfa v_{\tau+1} \geq 1-\epsilon_{\tau+1}:=  1-\frac{1}{2}\Big(\frac{\max_{i\in[\tau]}\delta_i+\sum_{i=1}^{\tau}\sqrt{8}\lambda_i\sqrt{\epsilon_i}}{\Delta}+\sqrt{2\epsilon_0}\Big)^2,
% \end{align*}
% and alternatively we have $\Vert\wha v_{\tau+1}-\bfa v_{\tau+1}\Vert_2\leq\sqrt{2\epsilon_{\tau+1}}$. Furthermore, consider the eigenvalue estimate, we show that
% \begin{align*}
%    \Big|\Big\Vert\Big(\bfa X\bfa X^\top-\sum_{i=1}^{\tau}\wh\lambda_i\wha v_i\wha v_i^\top\Big)\wha v_{\tau+1}\Big\Vert_2-\lambda_{\tau+1}\Big|\leq \frac{2\lambda_{\tau+1}}{\Delta}\Big(\max_{i\in[\tau]}\delta_i+\sum_{i=1}^{\tau}\sqrt{8}\lambda_i\sqrt{\epsilon_i}\Big)+\lambda_{\tau+1}\sqrt{2\epsilon_0}
% \end{align*}
% \end{lemma}

% \begin{lemma}[Approximation of norm by sum of Relu activations by Transformer networks]\label{reluapprox}
%     Assume that there exists a constant $C$ with $\Vert\bfa v\Vert_2\leq C$. There exists a multihead Relu attention layer with number of heads $M<\lef(\frac{\overline R}{\underline R}\rig)^d\frac{C(d)}{\epsilon^2}\log(1+C/\epsilon)$ such that there exsits $\{\bfa a_m\}_{m\in[M]}\subset\bb S^{N-1}$ and $\{c_m\}_{m\in[M]}\subset\bb R$ where for all $\bfa v$ with $\overline R\geq\Vert\bfa v\Vert_2\geq \underline R$, we have 
%     \begin{align*}
%         \bigg|\sum_{m=1}^Mc_m\sigma(\bfa a_m^\top\bfa v)-\frac{1}{\Vert\bfa v\Vert_2}+1\bigg|\leq\epsilon.
%     \end{align*}
%     Similarly, there exists a multihead Relu attention layer with number of heads $M\leq\overline R^{\frac{d}{2}}\frac{C(d)}{\epsilon^2}\log\lef(1+C/\epsilon\rig)$, a set of vectors $\{\bfa b_m\}_{m\in[M]}\subset\bb S^{N-1}$ and $\{d_m\}_{m\in[M]}\subset\bb R$ such that 
%     \begin{align*}
%         \Big|\sum_{m=1}^Md_m\sigma(\bfa b_m^\top\bfa v)-\Vert\bfa v\Vert_2^{1/2}+1\Big|\leq\epsilon.
%     \end{align*}
% \end{lemma}




